ViT-Lens: Towards Omni-modal Representations

Aiming to advance AI agents, large foundation models significantly improve reasoning and instruction execution, yet the current focus on vision and language neglects the potential of perceiving diverse modalities in open-world environments. However, the success of data-driven vision and language models is costly or even infeasible to be reproduced for rare modalities. In this paper, we present ViT-Lens-2 that facilitates efficient omni-modal representation learning by perceiving novel modalities with a pretrained ViT and aligning them to a pre-defined space. Specifically, the modality-specific lens is tuned to project any-modal signals to an intermediate embedding space, which are then processed by a strong ViT with pre-trained visual knowledge. The encoded representations are optimized toward aligning with the modal-independent space, pre-defined by off-the-shelf foundation models. ViT-Lens-2 provides a unified solution for representation learning of increasing modalities with two appealing advantages: (i) Unlocking the great potential of pretrained ViTs to novel modalities effectively with efficient data regime; (ii) Enabling emergent downstream capabilities through modality alignment and shared ViT parameters. We tailor ViT-Lens-2 to learn representations for 3D point cloud, depth, audio, tactile and EEG, and set new state-of-the-art results across various understanding tasks, such as zero-shot classification. By seamlessly integrating ViT-Lens-2 into Multimodal Foundation Models, we enable Any-modality to Text and Image Generation in a zero-shot manner. Code and models are available at https://github.com/TencentARC/ViT-Lens.

==> tab/tab_abla_tech_report.tex <==
\begin{table*}[t]
\caption{Ablation Study. We report top-1 zero-shot accuracy(\%) on ModelNet40.} \label{tab:abla-all}
\begin{subtable}[h]{0.37\textwidth}
\centering
\caption{More comparisons with PointBERT.}\label{tab:abla-3d-pointBERT}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|c|c}
\multicolumn{1}{l|}{PT.D::CLIP Model} & PointBERT & \methodname \\ \Xhline{3\arrayrulewidth}
\dsA :: OpenAI-B16      &    60.2       &     61.7      \\
\dsA :: Laion2B-B16     &    62.6       &     65.4      \\
\dsA :: OpenAI-L14      &    61.2       &     63.3      \\
\dsA :: Datacomp-L14    &    65.4       &     70.6      \\
\dsB :: OpenAI-B16      &    70.6       &     73.4      \\
\dsB :: Laion2B-B16     &    71.7       &     74.8      \\
\dsB :: OpenAI-L14      &    74.1       &     76.1      \\
\dsB :: Datacomp-L14    &    77.8       &     80.6      \\
\dsC :: bigG14          &    84.4       &     87.4          
\end{tabular}
}
}
\end{subtable}
\hfill
\begin{subtable}[h]{0.3\textwidth}
\centering
\caption{Configuration of Perceiver on depth and parameters sharing.}\label{tab:abla-perceiver}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{cc|c|c}
Depth & \begin{tabular}[c]{@{}c@{}}Share \\ Weights\end{tabular} & \#T.param & Acc@1 \\ \Xhline{3\arrayrulewidth}
2     &        -       &      34.1M    &  64.8     \\
4     &        \xmark     & 67.5M      &  64.2     \\
\rowcolor{lavenderweb}
4     &        \cmark     & 34.1M      &  65.4     \\
6     &         \xmark    & 100.8M     &  65.1     \\
6     &          \cmark   & 34.1M      &  64.0     \\
8     &          \xmark   & 134.2M     &  64.0     \\
8     &          \cmark   & 34.1M      &  64.3     \\
\end{tabular}
}
}
\end{subtable}
\hfill
\begin{subtable}[h]{0.3\textwidth}
\caption{Effect of Perceiver \#latents and ViT position embedding.}\label{tab:abla-hyperparam} % #num latent, use pt pos
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{cc|c|c}
\#latents & ViT.pos & Flops & Acc@1 \\ \Xhline{3\arrayrulewidth}
   128       &   \xmark      &   54.0G   &  65.1   \\
   128       &   \cmark      &   54.0G   &  65.2  \\
   196       &   \xmark      &  75.4G  & 65.1   \\
   \rowcolor{lavenderweb}
   196       &   \cmark      &  75.4G  & 65.4    \\
   256       &   \xmark      &  94.6G  & 65.5   \\
   256       &   \cmark      &  94.6G  & 65.5  \\
   384       &   \xmark      &  136.4G  & 66.2  \\
   384       &    \cmark     &  136.4G  &  66.3    \\
   512       &    \xmark     &  179.5G  &  66.3    \\
   512       &    \cmark     &  179.5G  &  67.4  
\end{tabular}
}
}
\end{subtable}
\\
\begin{subtable}[h]{0.45\textwidth}
\caption{``Point Embedding$\rightarrow$Perceiver'' Performance.}\label{tab:abla-point-perceiver} % #num latent, use pt pos
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{ccc|cc|c}
Depth & \#latents & \begin{tabular}[c]{@{}c@{}}Share \\ Weights\end{tabular} & \#T.param & Flops & Acc@1 \\ \Xhline{3\arrayrulewidth}
 2 & 196       &   -      &  34.1M   & 27.4G  & 62.2  \\
 4 & 196       &   \xmark      &  67.5M  & 40.5G  &  62.4  \\
 8 & 196       &   \xmark      & 134.6M   & 66.7G  & 62.7  \\
 6 & 196       &   \xmark      & 101.2M   & 53.6G  & 61.9  \\
 6 & 196       &   \cmark      & 34.1M   & 53.6G  &  62.3 \\
 6 & 256       &   \xmark      & 101.3M   & 65.6G &  63.5  \\
 6 & 256       &   \cmark      & 34.2M   & 65.6G &   62.7 \\
 6 & 512  &    \xmark     &  101.5M    & 116.6G   &  62.5  \\
 6 & 512  &    \cmark    & 34.4M    &  116.6G &  62.3 \\ \midrule
 \multicolumn{6}{l}{\textit{Default Settings} in \methodname} \\ \Xhline{2\arrayrulewidth}
 \rowcolor{lavenderweb}
 4 & 196  &    \cmark    & 34.1M  &  75.4G  &  65.4
\end{tabular}
}
}
\end{subtable}
\hfill
\begin{subtable}[h]{0.53\textwidth}
\caption{``Point Embedding$\rightarrow$\ptvit'' Performance.}\label{tab:abla-point-vit} % #num latent, use pt pos
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|cc|c}
\begin{tabular}[c]{@{}c@{}} Unlocked Components in \vit \end{tabular} & \#T.param & Flops & Acc@1 \\ \Xhline{3\arrayrulewidth}
% \multicolumn{4}{l}{\textit{\# transformer input tokens = 512}} \\ \Xhline{2\arrayrulewidth}
 None   &  7.3K  & 111.4G  &  50.0 \\
 \texttt{[CLS]}     &  7.3K  & 111.4G  &  53.6  \\
  \texttt{[CLS]}, \texttt{Proj}   & 1.1M   & 111.4G &  60.8  \\
  \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.1}, \texttt{Block.2}    & 15.3M     & 111.4G   &  64.8     \\
  \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.11}, \texttt{Block.12}  &  15.3M    & 111.4G   &  64.2    \\
  \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.1} - \texttt{Block.4}    & 29.5M     & 111.4G   &  65.4    \\
  \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.9} - \texttt{Block.12}    & 29.5M     & 111.4G   &  64.7    \\
  \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.1} - \texttt{Block.6}    & 43.7M     & 111.4G   &   66.4   \\
  \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.7} - \texttt{Block.12}    & 43.7M     & 111.4G   &  65.6    \\
  All & 86.6M  &  111.4G     &  67.7     \\ \midrule
  % \multicolumn{4}{l}{\textit{\# transformer input tokens = 196} } \\ \Xhline{2\arrayrulewidth}
  % \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.1}, \texttt{Block.2}    & 15.3M   &  40.4G    &   \\
  % \texttt{[CLS]}, \texttt{Proj}, \texttt{Block.11}, \texttt{Block.12}  &  15.3M    &  40.4G  &    \\
  %  All &   86.3M     &   40.4G          &       \\
  \multicolumn{4}{l}{\textit{Default Settings} in \methodname} \\ \Xhline{2\arrayrulewidth}
  \rowcolor{lavenderweb}
  None(tune PointEmb, Perceiver) & 34.1M & 75.4G &  65.4
\end{tabular}
}
}
\end{subtable}
\end{table*}

==> tab/tab_audio_cls.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|c|c|c|c|cc|cc}
\multirow{2}{*}{Method} & \multirow{2}{*}{anchor} & AudioSet & VGGSound  & ESC  & \multicolumn{2}{c|}{Clotho} & \multicolumn{2}{c}{AudioCaps} \\
                        &                         & mAP      & Top1      & Top1 & R@1          & R@10         & R@1           & R@10          \\ \hline
AVFIC                   & -                       & -        & -         & -    & 3.0          & 17.5         & 8.7           & 37.7          \\
ImageBind-H             & I                       & 17.6     & 27.8      & 66.9 & 6.0          & 28.4         & 9.3           & 42.3          \\
vitlensL                & I                       & 23.1     & 28.2      & 69.2 & 6.8          & 29.6         & 12.2          & 48.7          \\
AudioCLIP               & I+T                     & 25.9     & -         & 69.4 & -            & -            & -             & -             \\
vitlensL                & I+T                     & 26.7     & 31.7      & 75.9 & 8.1          & 31.2         & 14.4          & 52.6          \\
vitlensG                & I+T                     &          &           &      &              &              &               &               \\ \hline
Prev. ZS SOTA           & -                       & -        & 29.1/46.2 & 91.8 & 6.0          & 28.4         & 9.3           & 42.3   
\end{tabular}
}
\vspace{-0.5em}
\caption{Audio classification and retrieval on Audioset, VGGSound, ESC, Clotho and AudioCaps.}
\end{table}

==> tab/tab_audio_video.tex <==
\begin{table*}[h]
\centering
  \begin{minipage}{.63\textwidth} 
    \centering
        \resizebox{\textwidth}{!}{%
        \setlength{\tabcolsep}{4pt}
        \begin{tabular}{c|c|c|c|c|cc|cc}
        \multirow{2}{*}{\audioIcon{}} & \multirow{2}{*}{\textit{anchor}} & AudioSet & VGGSound$^\diamond$  & ESC$^\diamond$  & \multicolumn{2}{c|}{Clotho$^\diamond$} & \multicolumn{2}{c}{AudioCaps$^\diamond$} \\
                                &                         & mAP      & Top1      & Top1 & R@1          & R@10         & R@1           & R@10          \\ \Xhline{3\arrayrulewidth}
        \multicolumn{1}{l|}{AVFIC~\cite{nagrani2022avfic}}                 & -                       & -        & -         & -    & 3.0          & 17.5         & 8.7           & 37.7          \\
        \multicolumn{1}{l|}{ImageBind-H~\cite{girdhar2023imagebind}}          & I                       & 17.6     & 27.8      & 66.9 & 6.0          & 28.4         & 9.3           & 42.3          \\
        \multicolumn{1}{l|}{\vitlensL}                & I                       & 23.1     & 28.2      & 69.2 & 6.8          & 29.6         & 12.2          & 48.7          \\
        \multicolumn{1}{l|}{AudioCLIP~\cite{guzhov2022audioclip}}               & I+T                     & 25.9     & -         & 69.4 & -            & -            & -             & -             \\
        \multicolumn{1}{l|}{\vitlensL}                & I+T                     & \bf 26.7     & \bf 31.7      & \bf 75.9 & \bf 8.1          & \bf 31.2         & \bf 14.4          & \bf 54.9          \\ \hline
        % \vitlensG                & I+T                     &          &           &      &              &              &               &               \\ \hline
        \multicolumn{1}{l|}{Prev. ZS SOTA}           & -                       & -        & \color{DarkGray}29.1/46.2$^\star$~\cite{laionclap2023} & \color{DarkGray}91.8~\cite{wang2023onepeace} & 6.0          & 28.4~\cite{girdhar2023imagebind}         & 9.3       & 42.3~\cite{girdhar2023imagebind}   
        \end{tabular}
        }
        \vspace{-0.5em}
        \caption{Audio classification and retrieval on Audioset, VGGSound, ESC, Clotho and AudioCaps. $^\diamond$denotes zero-shot evaluation. {\color{DarkGray} Gray-out} denotes using larger audio-text datasets in pretraining. {\color{DarkGray}$^\star$}denotes using augmented captions for training.}\label{tab:audio_cls}
  \end{minipage}%
  \hfill
  \begin{minipage}{.345\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|c|ccc}
    \multicolumn{1}{c|}{\videoIcon{} \audioIcon{}}         & \textit{modality} & R@1  & R@5  & R@10 \\ \Xhline{3\arrayrulewidth}
    \color{DarkGray} MIL-NCE~\cite{miech2019howto100m} & \color{DarkGray} V & \color{DarkGray} 8.6 & \color{DarkGray} 16.9 & \color{DarkGray} 25.8 \\
    \color{DarkGray} SupportSet~\cite{patrick2021supportset} & \color{DarkGray} V & \color{DarkGray} 10.4 & \color{DarkGray} 22.2 & \color{DarkGray} 30.0 \\
    \color{DarkGray} AVFIC~\cite{nagrani2022avfic}          & \color{DarkGray} A+V      & \color{DarkGray} 19.4 & \color{DarkGray} 39.5 & \color{DarkGray} 50.3 \\
    ImageBind-H~\cite{girdhar2023imagebind}    & A+V      & 36.8 & 61.8 & 70.0 \\
    \vitlensL       & A+V      & \bf 37.6 & \bf 63.2 & \bf 72.6 \\ \hline
    % \vitlensG       & A+V      & \bf 37.9 & \bf 64.0 & \bf 73.2 \\ \hline
    \color{DarkGray}Zero-shot SOTA~\cite{chen2023vast} & \color{DarkGray}V        & \color{DarkGray}49.3 & \color{DarkGray}68.3 & \color{DarkGray}73.9
    \end{tabular}
    }
    \vspace{-0.5em}
    \caption{Video Retrieval on MSRVTT. V: use video; A+V: use audio and video. {\color{DarkGray}Gray-out} means using video data in pretraining.}\label{tab:video_ret}
  \end{minipage}
  \vspace{-0.2em}
\end{table*}

==> tab/tab_depth_cls.tex <==
\begin{table}[h]
\centering
\resizebox{0.75\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|c|cc}
Method      & \textit{anchor} & NYU-D & SUN-D \\ \Xhline{2\arrayrulewidth}
Text Paired~\cite{girdhar2023imagebind} & T*     & 41.9  & 25.4  \\
ImageBind-H~\cite{girdhar2023imagebind} & I      & 54.0  & 35.1  \\
\vitlensL    & I      & 64.2  & 37.4  \\
\vitlensL    & I+T     & 68.5  & 52.2  \\
\vitlensG    & I+T     & 69.4  & 54.5  \\ \hline
\color{DarkGray} supervised SOTA~\cite{girdhar2022omnivore} &  
\color{DarkGray}-   & \color{DarkGray} 76.7  & \color{DarkGray} 64.9
\end{tabular}
}
\vspace{-0.5em}
\caption{Depth-only scene classification on NYU-D and SUN-D.}\label{tab:depth_cls}
\end{table}

==> tab/tab_depth_tactile_eeg.tex <==
\begin{table*}[th] % You can place it inside a table environment to add a caption and label
  \centering
  \begin{minipage}{.33\textwidth} % Each minipage takes 25% of the text width
    \centering
    \resizebox{\textwidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{l|c|cc}
        \multicolumn{1}{c|}{\depthIcon{}}      & \textit{anchor} & NYU-D & SUN-D \\ \Xhline{3\arrayrulewidth}
        Text Paired~\cite{girdhar2023imagebind} & T$^\star$     & 41.9  & 25.4  \\
        ImageBind-H~\cite{girdhar2023imagebind} & I      & 54.0  & 35.1  \\
        \vitlensL    & I      & 64.2  & 37.4  \\
        \vitlensL    & I+T     & \bf 68.5  & \bf 52.2  \\ \hline
        % \vitlensG    & I+T     & \bf 69.4  & \bf 54.5  \\ \hline
        \color{DarkGray} Supervised SOTA~\cite{girdhar2022omnivore} &  
        \color{DarkGray}-   & \color{DarkGray} 76.7  & \color{DarkGray} 64.9
        \end{tabular}
    }
        \vspace{-0.5em}
        \caption{Depth-only scene classification on NYU-D and SUN-D. $^\star$\cite{girdhar2023imagebind} rendered depth as grayscale images for direct testing. The supervised SOTA~\cite{girdhar2022omnivore} used RGBD as input and extra training data.}\label{tab:depth_cls}
  \end{minipage}%
  \hfill
  \begin{minipage}{.315\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{l|c|ccc}
        \multicolumn{1}{c|}{\tactileIcon{}}                   & \textit{anchor} & Material & H/S & R/S \\ \Xhline{3\arrayrulewidth}
        ImageBind-B$^\ast$             & I      & 24.2     & 65.7      & 69.8                             \\
        \vitlensB                 & I      & 29.9     & 72.4   & 77.9                           \\
        \vitlensL                 & I      &  31.2        &    74.3       &         \bf 78.2                        \\
        \vitlensL                 & I+T     &  \bf 65.8       &    \bf 74.7       &          63.8                        \\ \hline
        \multicolumn{5}{l}{\textit{Linear Probing}} \\
        CMC~\cite{tian2020cmc,yang2022touch_and_go}                      & I      & 54.7     & 77.3      & 79.4                             \\
        \vitlensB  & I      & \bf 63.0     & \bf 92.0      & \bf 85.1               
        \end{tabular}
    }
        \vspace{-0.5em}
        \caption{Tactile classification on Touch-and-go. $^\ast$denotes our implementation. H/S: Hard/Soft; R/S: Rough/Smooth.}\label{tab:tactile_cls}
  \end{minipage}%
  \hfill
  \begin{minipage}{.32\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
        \setlength{\tabcolsep}{3pt}
        \begin{tabular}{l|c|cc}
        \multicolumn{1}{c|}{\eegIcon{}}           & \textit{anchor} & Val  & Test \\ \Xhline{3\arrayrulewidth}
        ImageBind-B$^\ast$      & I      & 17.3 & 18.4 \\
        DreamDiffusion-L\textsuperscript{\#}~\cite{bai2023dreamdiffusion} & I      & 20.4 & 19.2 \\
        \vitlensB         & I      & 24.6 & 25.3 \\
        \vitlensL         & I      &  29.3    &   29.2   \\
        \vitlensL         & I+T     & \bf 41.8 & \bf 42.7
        \end{tabular}
    }
\vspace{-0.5em}
\caption{Visual concept classification on ImageNet-EEG. $^\ast$denotes our implementation. \textsuperscript{\#}We use the released EEG encoder and paired text encoder for inference. We report results on Val and Test set.}\label{tab:eeg_cls}
  \end{minipage}%
\vspace{-0.5em}
\end{table*}

==> tab/tab_eeg_cls.tex <==
\begin{table}[h]
\centering
\resizebox{0.65\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|c|cc}
Method           & \textit{anchor} & Val  & Test \\ \Xhline{2\arrayrulewidth}
ImageBind-B*     & I      & 17.3 & 18.4 \\
DreamDiffusion-L~\cite{bai2023dreamdiffusion} & I      & 20.4 & 19.2 \\
\vitlensB         & I      & 24.6 & 25.3 \\
\vitlensL         & I      &      &      \\
\vitlensL         & I+T     & 41.8 & 42.7
\end{tabular}
}
\vspace{-0.5em}
\caption{Visual concept classification on ImageNet-EEG.}
\end{table}

==> tab/tab_mllm_example_toilet.tex <==
\begin{table*}[h]
\begin{minipage}{0.99\textwidth}
\centering  
\scalebox{0.88}{
\begin{tabular}{l p{10.5cm} }
\toprule
 \multicolumn{2}{l}{\bf Visual input example, Toilet:}  \\
\midrule
&  \includegraphics[height=3.5cm]{fig/toilet_0375_crop.png} \\

User & What is in the scene? \\
InstructBLIP w/ \methodname & Toilet.\\
User & Describe it in detail. \\
InstructBLIP w/ \methodname & The image features a close-up view of a toilet with its lid open, revealing the inside of the toilet bowl. The toilet appears to be made of porcelain or ceramic material, and it has a seat attached to it. The toilet is positioned on a white background, providing a clear and detailed view of the toilet's design and construction. In addition to the toilet, there is another object in the image, which could be a piece of furniture or a decorative item, but it is not as prominent as the toilet. Overall, the image showcases a functional and well-designed toilet, emphasizing the importance of cleanliness and hygiene in daily life.
\\
\midrule
User & What is in the scene? \\
InstructBLIP w/ PointBERT &  Lamp. \\
User & Describe this object briefly. \\
InstructBLIP w/ PointBERT & An image of a desk with a lamp on it. \\
\midrule
CLIPCap-Openshape~\cite{mokady2021clipcap,liu2023openshape} & The moment a man's hand reaches out to touch a toilet bowl. \\
\bottomrule
\end{tabular}
}
\captionof{table}{Example for \methodname enabling InstructBLIP to understand 3D inputs.}  
\label{tab:visual_example_toilet} 
\end{minipage}
\end{table*}

==> tab/tab_tactile_cls.tex <==
\begin{table}[h]
\centering
\resizebox{0.95\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|c|ccc}
Method                   & \textit{anchor} & Material & Hard/Soft & \multicolumn{1}{l}{Rough/Smooth} \\ \Xhline{2\arrayrulewidth}
ImageBind-B*             & I      & 24.2     & 65.7      & 69.8                             \\
\vitlensB                 & I      & 29.9     & 72.4      & 77.9                             \\
\vitlensL                 & I      &          &           &                                  \\
\vitlensL                 & I+T     &          &           &                                  \\ \hline
\multicolumn{5}{l}{\textit{Linear Probe}} \\
CMC~\cite{yang2022touch_and_go}                      & I      & 54.7     & 77.3      & 79.4                             \\
\vitlensB $\rightarrow$ I & I      & 63.0     & 92.0      & 85.1               
\end{tabular}
}
\vspace{-0.5em}
\caption{Tactile related classification on Touch-and-go.}
\end{table}

==> tab/tab_video_retrieval.tex <==
\begin{table}[h]
\centering
\resizebox{0.75\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|c|ccl}
Method         & Modality & R@1  & R@5  & R@10 \\ \Xhline{2\arrayrulewidth}
AVFIC~\cite{nagrani2022avfic}          & A+V      & 19.4 & 39.5 & 50.3 \\
ImageBind-H~\cite{girdhar2023imagebind}    & A+V      & 36.8 & 61.8 & 70.0 \\
\vitlensL       & A+V      & 37.6 & 63.2 & 72.6 \\
\vitlensG       & A+V      & 37.9 & 64.0 & 73.2 \\ \hline
\color{DarkGray}Zero-shot SOTA~\cite{chen2023vast} & \color{DarkGray}V        & \color{DarkGray}49.3 & \color{DarkGray}68.3 & \color{DarkGray}73.9
\end{tabular}
}
\vspace{-0.5em}
\caption{Video Retrieval on MSRVTT.}
\end{table}
